On Memory Construction and Retrieval for Personalized Conversational Agents

To deliver coherent and personalized experiences in long-term conversations, existing approaches typically perform retrieval augmented response generation by constructing memory banks from conversation history at either the turn-level, session-level, or through summarization techniques.In this paper, we present two key findings: (1) The granularity of memory unit matters: turn-level, session-level, and summarization-based methods each exhibit limitations in both memory retrieval accuracy and the semantic quality of the retrieved content. (2) Prompt compression methods, such as LLMLingua-2, can effectively serve as a denoising mechanism, enhancing memory retrieval accuracy across different granularities. Building on these insights, we propose SeCom, a method that constructs the memory bank at segment level by introducing a conversation segmentation model that partitions long-term conversations into topically coherent segments, while applying compression based denoising on memory units to enhance memory retrieval. Experimental results show that SeCom exhibits a significant performance advantage over baselines on long-term conversation benchmarks LOCOMO and Long-MT-Bench+. Additionally, the proposed conversation segmentation method demonstrates superior performance on dialogue segmentation datasets such as DialSeg711, TIAGE, and SuperDialSeg.

==> tables/main_comp_comp.tex <==
\begin{table*}[!t]
    \small
    \centering
    \setlength{\tabcolsep}{1mm}
    % \vspace{-2ex}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{l|cccccc|cc}
    \toprule
    
    \multirow{2}{*}{\textbf{Methods}} &  \multicolumn{6}{@{}c|}{{\bf QA Performance}} & \multicolumn{2}{@{}c}{{\bf Length}} \\
    \cmidrule (lr){2-7} \cmidrule (lr){8-9}
    & GPT4Score & BLEU & Rouge1 & Rouge2 & RougeL & BERTScore & \# Turns & \# Tokens \\
    \midrule
    \multicolumn{9}{@{}c}{{ \texttt{GPT-35} }} \\
    \midrule
    Round-Level & 84.91 & 17.01 & 38.01 & 23.88 & 31.59 & 88.64 & 3.00 & 911 \\
    Session-Level & 63.38 & 12.22 & 28.89 & 14.98 & 22.94 & 86.64 & 13.38 & 3,613 \\
    Full History & 53.85 & 5.63 & 20.69 & 8.49 & 15.83 & 84.82 & 65.45 & 19,288 \\
    \midrule
    Segment (Origin) & 88.81 & \textbf{18.02} & \textbf{39.48} & \textbf{24.93} & \textbf{33.54} & \textbf{88.81} & 2.78 & 811 \\
    \midrule
    Segment (Comp. n=1) & 86.69 & 15.81 & 39.06 & 23.08 & 32.65 & 88.51 & 2.78 & 630 \\
    Segment (Comp. n=2) & \textbf{89.73} & 16.40 & 39.39 & 24.03 & 33.10 & 88.50 & 5.40 & 1,172 \\

    \midrule
    \multicolumn{9}{@{}c}{{ \texttt{Mistral-7B-v0.3} }} \\
    \midrule
    Round-Level & 86.02 & 17.25 & 40.35 & 25.21 & 33.45 & 88.73 & 3.00 & 911 \\
    Session-Level & 68.04 & 8.25 & 30.26 & 16.63 & 23.79 & 86.66 & 13.38 & 3,613 \\
    Full History & 80.07 & 6.15 & 27.55 & 15.45 & 21.87 & 86.22 & 65.45 & 19,288 \\
    \midrule
    Segment (Origin) & \textbf{90.42} & \textbf{17.71} & 41.18 & \textbf{25.98} & 34.63 & \textbf{88.88} & 2.78 & 811 \\
    \midrule
    Segment (Comp. n=1) & - & 16.83 & \textbf{41.83} & 24.81 & \textbf{34.73} & 88.85 & 2.78 & 630 \\
    Segment (Comp. n=2) & - & 15.29 & 40.60 & 24.04 & 33.71 & 88.57 & 5.40 & 1,172 \\
    
    \bottomrule
    \end{tabular}
    }
    \caption{The evaluation results on the \textit{Long-MT-Bench+}, ``Comp. n=1" denotes retrieving the top n segments to the response generator. 
    }
    \label{tab: main_llmlingua2}
\end{table*}

==> tables/ours_vs_memochat.tex <==
\begin{table}[t]
    \small
    \centering
    \setlength{\tabcolsep}{1mm}
    \resizebox{1\columnwidth}{!}{
    \begin{tabular}{l|cccc}
    \toprule

    \textbf{Methods} & \# In. Token & \# Out. Token & Latency (s) & GPT Score \\
    \midrule
    
    \multicolumn{5}{@{}c}{{ \textit{LOCOMO} }} \\
    \midrule
    MemoChat & 683,085 & 9,711 & 1155.62 & 65.10 \\ 
    Ours & 29,639 & 5,031 & 256.60 & \textbf{69.33} \\ 
    \midrule
    \multicolumn{5}{@{}c}{{ \textit{Long-MT-Bench+} }} \\
    \midrule
    MemoChat & 145,836 & 3,328 & 564.54 & 85.14 \\ 
    Ours & 23,027 & 1,741 & 122.42 & \textbf{88.81} \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Comparison between our method and \textit{MemoChat} from multiple aspects. ``\# In. Token", ``\# Out. Token" and ``Latency" report the number of input / output token and the latency per sample.}
    \label{tab: ours_vs_memochat}
\end{table}

==> tables/segment_dialseg.tex <==
\begin{table*}[ht]
    \small
    \centering
    % \setlength{\tabcolsep}{1mm}
    % \vspace{-2ex}
    \resizebox{\columnwidth}{!}{
    
    \begin{tabular}{ccccc|ccccc}
    \toprule
    \multicolumn{5}{@{}c|}{{\bf Unsupervised}} & \multicolumn{5}{@{}c}{{\bf Supervised Learning on SuperDialSeg}} \\
    \cmidrule (lr){1-5} \cmidrule (lr){6-10}
    Methods & Pk↓ & WD↓ & F1↑ & Score↑ & Methods & Pk↓ & WD↓ & F1↑ & Score↑ \\
    \midrule
    
    BayesSeg & 0.306 & 0.350 & 0.556 & 0.614 & $\text{TextSeg}_{dial}$ & 0.453 & 0.461 & 0.367 & 0.455 \\
    CSM & 0.278 & 0.302 & \underline{0.610} & \underline{0.660} & BERT & 0.401 & 0.473 & 0.381 & 0.472 \\
    DialSTART $^{\dag}$ & \underline{0.178} & \underline{0.198} & - & - & RoBERTa & \underline{0.241} & \underline{0.272} & \underline{0.660} & \underline{0.702} \\
    
    \midrule
    \textbf{Ours (zero-shot)} & \textbf{0.093} & \textbf{0.103} & \textbf{0.888} & \textbf{0.895} & \textbf{Ours (few-shot)} & \textbf{0.049} & \textbf{0.054} & \textbf{0.924} & \textbf{0.936} \\
    
    \bottomrule
    \end{tabular}
    }
    \caption{Segment performance on Dialseg711.
    $^{\dag}$: numbers reported in \citet{gao2023unsupervised}. Other baselines are reported in \citet{jiang2023superdialseg}.}
    \label{tab: segment_dialseg}
    \vspace{-3mm}
\end{table*}


==> tables/unsupervised_segment.tex <==
\begin{table*}[t]
    \small
    \centering
    \setlength{\tabcolsep}{1mm}
    \caption{Segmentation performances on three datasets.
    $^{\dag}$: numbers reported in \citet{gao2023unsupervised}. Other baselines are reported in \citet{jiang2023superdialseg}. The best performance is highlighted in \textbf{bold}, and the second best is highlighted by \underline{underline}. \colorbox{light_gray}{Numbers in gray} correspond to \textbf{supervised} setting.}
    \label{tab: segment_main}
    \resizebox{\columnwidth}{!}{
    
    \begin{tabular}{l|cccc|cccc|cccc}
    \toprule
    \multirow{2}{*}{\textbf{Methods}} & \multicolumn{4}{@{}c}{{\bf Dialseg711}} & \multicolumn{4}{@{}c}{{\bf SuperDialSeg}} & \multicolumn{4}{@{}c}{{\bf TIAGE}}  \\
    \cmidrule (lr){2-5} \cmidrule (lr){6-9} \cmidrule (lr){10-13} 
    & Pk↓ & WD↓ & F1↑ & Score↑ & Pk↓ & WD↓ & F1↑ & Score↑ & Pk↓ & WD↓ & F1↑ & Score↑ \\

    \midrule
    \multicolumn{13}{@{}c}{\textbf{Unsupervised}} \\
    \midrule
    
    BayesSeg & 0.306 & 0.350 & 0.556 & 0.614 & \underline{0.433} & 0.593 & \underline{0.438} & 0.463 & 0.486 & 0.571 & 0.366 & 0.419\\
    TextTiling & 0.470 & 0.493 & 0.245 & 0.382 & 0.441 & \underline{0.453} & 0.388 & \underline{0.471} & 0.469 & 0.488 & 0.204 & 0.363 \\
    GraphSeg & 0.412 & 0.442 & 0.392 & 0.483 & 0.450 & 0.454 & 0.249 & 0.398 & 0.496 & 0.515 & 0.238 & 0.366\\
    \midrule
    TextTiling+Glove & 0.399 & 0.438 & 0.436 & 0.509 & 0.519 & 0.524 & 0.353 & 0.416 & 0.486 & 0.511 & 0.236 & 0.369\\
    TextTiling+[CLS] & 0.419 & 0.473 & 0.351 & 0.453 & 0.493 & 0.523 & 0.277 & 0.385 & 0.521 & 0.556 & 0.218 & 0.340 \\
    TextTiling+NSP & 0.347 & 0.360 & 0.347 & 0.497 & 0.512 & 0.521 & 0.208 & 0.346 & 0.425 & 0.439 & 0.285 & 0.426\\
    GreedySeg & 0.381 & 0.410 & 0.445 & 0.525 & 0.490 & 0.494 & 0.365 & 0.437 & 0.490 & 0.506 & 0.181 & 0.341\\
    CSM & 0.278 & 0.302 & \underline{0.610} & \underline{0.660} & 0.462 & 0.467 & 0.381 & 0.458 & \underline{0.400} & \underline{0.420} & \underline{0.427} & \underline{0.509} \\
    DialSTART $^{\dag}$ & \underline{0.178} & \underline{0.198} & - & - & - & - & - & - & - & - & - & - \\
    \midrule
    \textbf{Ours} & \textbf{0.093} & \textbf{0.103} & \textbf{0.888} & \textbf{0.895} & \textbf{0.277} & \textbf{0.289} & \textbf{0.758} & \textbf{0.738} & \textbf{0.363} & \textbf{0.401} & \textbf{0.596} & \textbf{0.607} \\
    
    \bottomrule
    \end{tabular}
    }
\end{table*}

